Logic-guided Semantic Representation Learning for Zero-Shot Relation Classification

Relation classification aims to extract semantic relations between entity pairs from the sentences. However, most existing methods can only identify seen relation classes that occurred during training. To recognize unseen relations at test time, we explore the problem of zero-shot relation classification. Previous work regards the problem as reading comprehension or textual entailment, which have to rely on artificial descriptive information to improve the understandability of relation types. Thus, rich semantic knowledge of the relation labels is ignored. In this paper, we propose a novel logic-guided semantic representation learning model for zero-shot relation classification. Our approach builds connections between seen and unseen relations via implicit and explicit semantic representations with knowledge graph embeddings and logic rules. Extensive experimental results demonstrate that our method can generalize to unseen relation types and achieve promising improvements.

==> data_wiki.tex <==
\begin{table}[htb]
\centering
% \small
\normalsize
% \large
\caption{Statistics of the dataset}\label{dataset_wiki}
\linespread{1.3}\selectfont
\begin{tabular}{c|c|c|c|c}
% \hline
\Xhline{1.2pt}
			\hline
            Dataset & \#Rel(seen) & \#Rel(unseen) & \#Sent & \#Fact\\
            \hline
            Training &  &  &  &\\
            Validation &  &  &  &\\
            Test &  &  &  &\\
\Xhline{1.2pt}
% \hline
\end{tabular}
\end{table}

==> table2.tex <==
\begin{table*}
\centering
    \small
\begin{tabular}{c | c | c | c | c}
%=============== Part 1 ====================
\Xhline{1.0pt}
\textbf{Unseen Relations} 
& \multicolumn{2}{|c}{\textbf{lyrics\_by}}
& \multicolumn{2}{|c}{\textbf{after\_a\_work\_by}}\\
\hline
F1-score
& +$E_{kg}$: 0.52
& $E_{wd}$: 0.01 
& +$E_{kg}$: 0.51
& $E_{wd}$: 0.01 \\

\hline

\multirow{3}{*}{Top3 relations} 
& performer
& influenced\_by 
& author
& named\_after \\

%\multirow{3}{*}{Top3 related seen relations} 
& composer
& spouse 
& screenwriter
& author \\

%\multirow{3}{*}{Top3 related seen relations} 
& cast\_member
& cast\_member
& creator
& characters \\

%================Part 2===================
\Xhline{1.0pt}

\textbf{Unseen Relations} 
& \multicolumn{2}{|c}{\textbf{location\_of\_formation}}
& \multicolumn{2}{|c}{\textbf{residence}}\\
\hline
F1-score 
& +$E_{kg}$: 0.46
& $E_{wd}$: 0.02 
& +$E_{kg}$: 0.36
& $E_{wd}$: 0.01 \\

\hline

\multirow{3}{*}{\shortstack{Top3 relations}} 
& headquarters\_location
& subclass\_of 
& place\_of\_death
& twinned administration \\

%\multirow{3}{*}{Top3 related seen relations} 
& location
& opposite\_of 
& place\_of\_birth
& place\_of\_death \\

%\multirow{3}{*}{Top3 related seen relations} 
& capital
& part\_of
& educated\_at
& place\_of\_birth \\

%===============Part 3====================
\Xhline{1.0pt}

\textbf{Unseen Relations} 
& \multicolumn{2}{|c}{\textbf{work\_location}}
& \multicolumn{2}{|c}{\textbf{occupant}}\\
\hline
F1-score 
& +$E_{kg}$: 0.40
& $E_{wd}$: 0.05 
& +$E_{kg}$: 0.31
& $E_{wd}$: 0.00 \\

\hline

\multirow{3}{*}{Top3 relations} 
& place\_of\_death
& place\_of\_death 
& owned by
& -- \\

%\multirow{3}{*}{Top3 related seen relations} 
& place\_of\_birth
& headsquarters\_location 
& location 
& -- \\

%\multirow{3}{*}{Top3 related seen relations} 
& headsquarters\_location
& twinned administration
& headsquarters\_location
& -- \\

\Xhline{1.0pt}	
\end{tabular}
\caption{
    	% 说明下top3的排名
    	% 说明空白表示样本被预测到对应关系上
    	}
    	\vspace{-6mm}
\end{table*}


% \begin{table*}[!htb]
%     \centering
%     \small
%     \begin{tabular} {p{90pt}|c|c|p{102pt}|p{125pt}}
%     	\Xhline{1.2pt}

%     	\multirow{2}{*}{\shortstack{Unseen Relations}}& \multicolumn{2}{|c|}{F1-score} & \multicolumn{2}{|c}{Top $3$ related seen relations}\\ \cline{2-5}
%     	& \multicolumn{1}{|c|}{+$E_{kg}$} & \multicolumn{1}{|c|}{ +$E_{wd}$} & \multicolumn{1}{|c|}{ +$E_{kg}$ } & \multicolumn{1}{|c}{+$E_{wd}$} \\	
% 		\Xhline{0.8pt}

% 		\multirow{3}{*}{lyrics\_by} & \multirow{3}{*}{0.52}& \multirow{3}{*}{0.01}   & performer &influenced\_by \\ \cline{4-5}
%     	&&& composer &spouse \\ \cline{4-5}
% 		&&& cast\_member &cast\_member \\
% 		\Xhline{0.8pt}
		
% 		\multirow{3}{*}{after\_a\_work\_by}  & \multirow{3}{*}{0.51}& \multirow{3}{*}{0.01}  & author & named\_after \\ \cline{4-5}
%     	&&& screenwriter & author \\ \cline{4-5}
% 		&&& creator & characters \\ 
% 		\Xhline{0.8pt}

% 		\multirow{3}{*}{\shortstack{location\_of\_formation}}& \multirow{3}{*}{0.46}& \multirow{3}{*}{0.02} & headquarters\_location & subclass\_of \\ \cline{4-5}
%     	&&& location & opposite\_of\\ \cline{4-5}
% 		&&& capital & part\_of \\ 
% 		\Xhline{0.8pt}

% 		\multirow{3}{*}{residence} & \multirow{3}{*}{0.36} & \multirow{3}{*}{0.01} & place of death & twinned administrative body \\ \cline{4-5}
%     	&&& place\_of\_birth & place\_of\_death\\ \cline{4-5}
% 		&&& educated\_at & place\_of\_birth \\ 
% 		\Xhline{0.8pt}

% 		\multirow{3}{*}{work\_location} & \multirow{3}{*}{0.40} & \multirow{3}{*}{0.05}   & place\_of\_death & place\_of\_death\\ \cline{4-5}
% 		&&& place\_of\_birth & headquarters\_location \\ \cline{4-5}
%     	&&& headquarters\_location & twinned\_administrative\_body \\
%     	\Xhline{0.8pt}
		
% 	  	\multirow{3}{*}{mother} & \multirow{3}{*}{0.81}  & \multirow{3}{*}{0.50}  &follows &child  \\ \cline{4-5}
% 		&&& spouse  &spouse   \\ \cline{4-5}
%     	&&& twinned administrative body  &father   \\ \hline
%     	\Xhline{0.8pt}

    	
% 		\multirow{3}{*}{producer} & \multirow{3}{*}{0.54}  & \multirow{3}{*}{0.43}  &director &screenwriter  \\ \cline{4-5}
% 		&&&screenwriter   &director   \\ \cline{4-5}
%     	&&&cast member  &cast member   \\ \hline
%     	\Xhline{0.8pt}

% 		\multirow{3}{*}{nominated\_for} & \multirow{3}{*}{0.96}  & \multirow{3}{*}{0.52}  & award\_received&award\_received  \\ \cline{4-5}
% 		&&&educated\_at   &part\_of   \\ \cline{4-5}
%     	&&&participant\_of&member\_of   \\ \hline
%     	\Xhline{0.8pt}

% 	  	\multirow{3}{*}{crosses} & \multirow{3}{*}{0.58}  & \multirow{3}{*}{0.23}  &mouth of the watercourse&mouth of the watercourse \\ \cline{4-5}
% 		&&&located in or next to body of water &located in or next to body of water  \\ \cline{4-5}
%     	&&&located on terrain feature  & located on terrain feature \\ 
%     	\Xhline{0.8pt}


% 		\multirow{3}{*}{office contested} & \multirow{3}{*}{0.26}  & \multirow{3}{*}{0.00}  &position held &  \\ \cline{4-4}
% 		&&&successful candidate& \quad\quad\quad\quad--------------  \\ \cline{4-4}
%     	&&&applies to jurisdiction   &  \\ \hline
%     	\Xhline{0.8pt}

%     	\multirow{3}{*}{occupant}  & \multirow{3}{*}{0.31} & \multirow{3}{*}{0.00}  &owned by& \multirow{3}{*}{\quad\quad\quad\quad--------------} \\ \cline{4-4}
% 		&&&location  &  \\ \cline{4-4}
%     	&&&headquarters\_location&  \\ 
%     	\Xhline{0.8pt}

%     	\multirow{3}{*}{drafted\_by}  & \multirow{3}{*}{0.81} & \multirow{3}{*}{0.01}  & member\_of sports\_team & \multirow{3}{*}{\quad\quad\quad\quad--------------}  \\ \cline{4-4}
%     	&&& educated\_at & \\ \cline{4-4}
% 		&&& member\_of & \\ 
%     	% \Xhline{0.8pt}
						

%   %   	\multirow{3}{*}{} & \multirow{3}{*}{0.}  & \multirow{3}{*}{0.}  & &  \\ \cline{4-5}
% 		% &&&   &   \\ \cline{4-5}
%   %   	&&&   &   \\ \hline

% 		% \multirow{3}{*}{} & \multirow{3}{*}{0.}  & \multirow{3}{*}{0.}  & &  \\ \cline{4-5}
% 		% &&&   &   \\ \cline{4-5}
%   %   	&&&   &   \\ \hline

%     	\Xhline{1.0pt}


  
% 	% \multirow{3}{*}{deepest point } & \multirow{3}{*}{0.49} & \multirow{3}{*}{0.19}  & located in or next to body of water &located on terrain feature \\ \cline{4-5}
% 		% &&&located on terrain feature  & located in or next to body of water  \\ \cline{4-5}
%   %   	&&&mouth of the watercourse  & continent \\ 
%   %   	\hline
%     \end{tabular}
%     \caption{
%     	% 说明下top3的排名
%     	% 说明空白表示样本被预测到对应关系上
%     	}
% \end{table*}

==> tables/zslp-case.tex <==
\begin{table}[htb]
\centering
\caption{Cases zslp}\label{zslp case}
\linespread{1.3}\selectfont
\begin{tabular}{c|c|c|c|l}
\hline
Relation                & $E_{wd}$              & $E_{kg}$              & $E_{rl}$              & Rules \\
\hline
\multirow{3}{*}{xxx}    & \multirow{3}{*}{A}    & \multirow{3}{*}{B}    & \multirow{3}{*}{C}    & 1     \\\cline{5-5}
                        &                       &                       &                       & 2     \\\cline{5-5}
                        &                       &                       &                       & 3     \\
\hline
\multirow{3}{*}{xxx}    & \multirow{3}{*}{A}    & \multirow{3}{*}{B}    & \multirow{3}{*}{C}    & 1     \\\cline{5-5}
                        &                       &                       &                       & 2     \\\cline{5-5}
                        &                       &                       &                       & 3     \\
\hline
\multirow{3}{*}{xxx}    & \multirow{3}{*}{A}    & \multirow{3}{*}{B}    & \multirow{3}{*}{C}    & 1     \\\cline{5-5}
                        &                       &                       &                       & 2     \\\cline{5-5}
                        &                       &                       &                       & 3     \\
\hline
\end{tabular}
\end{table}

==> tables/zslp-general.tex <==
\begin{table*}[htb]
\label{zslp general}
\centering
\caption{The result of ZSLP under GZSL.}\label{zslp gzsl}
\linespread{1.3}\selectfont
\begin{tabular}{c|ccccccccc}
\hline
            &$MRR^{S}$  &$Hit_{1}^{S}$ & $Hit_{5}^{S}$  &$MRR^{U}$  &$Hit_{1}^{U}$ &$Hit_{5}^{U}$  &$H_{MRR}$   &$H_{1}$  &$H_{5}$\\
\hline
$E_{rand}$    &94.93	&92.29	&98.86 &2.98	&0.28	&1.83 &5.79	&0.55	&3.59\\
\hline
$E_{kp}$    &95.59	&93.29	&99.43	&17.98	&4.16	&10.72	&41.01	&26.31	&57.80  \\
$E_{rpk}$   &89.64	&85.00	&94.71	&36.50	&20.87	&54.38	&51.88	&33.51	&69.09  \\
$E_{pk}$    &92.93	& 89.71	 & 98.00 & \textbf{41.30}	 &\textbf{ 28.01}	 & \textbf{58.26} & \textbf{57.18}	 & \textbf{42.69}	 & \textbf{73.08 }    \\
\hline
\end{tabular}
\end{table*}

==> tables/zslp-traditional.tex <==
\begin{table}[htb]
\label{zslp traditional}
\centering
\caption{The result of ZSLP under TZSL.}\label{tab2}
\linespread{1.3}\selectfont
\begin{tabular}{c|cccc}
\hline
&$MRR$  &$Hit_{1}$  &$Hit_{2}$  &$Hit_{5}$\\
\hline
$E_{rand}$ &15.35	&4.84	&8.43	&19.97\\
\hline
$E_{kp}$  &60.25	&46.56	&61.16	&76.41\\
$E_{rpk}$ &60.47	&47.99	&59.31	&76.37\\
$E_{pk}$  &\textbf{62.62}	&\textbf{49.70}	&\textbf{63.08}	&\textbf{78.02}\\
\hline
\end{tabular}
\end{table}

==> tables/zsre-case.tex <==
% \include{explanation_rule.tex}

\begin{table*}[htb]
	\label{zsre case}
	\centering
	\small
	% \begin{tabular}{p{67pt}|p{25pt}|p{25pt}|p{25pt}|p{280pt}}

	\begin{tabular}{l|p{0.55cm}<{\centering}|p{0.55cm}<{\centering}|p{0.55cm}<{\centering}|p{0.55cm}<{\centering}|p{0.55cm}<{\centering}|p{0.55cm}<{\centering}|l}
		\Xhline{1.2pt}
		  \multirow{2}{*}{\shortstack{Unseen\\Relations}} & \multicolumn{6}{c|}{$acc_1$} & \multirow{2}{*}{ Related rules w.r.t. unseen relations}\\ \cline{2-7} &+$E_{wd}$ &+$E_{kg}$ &+$E_{rl}$ & +$E_{wk}$ & +$E_{wr}$ &+$E_{kr}$ & \\ 
      \Xhline{0.8pt}


         \multirow{3}{*}{producer} & \multirow{3}{*}{54.0}   &
      \multirow{3}{*}{71.14}  & \multirow{3}{*}{68.71}&
      \multirow{3}{*}{48.43}   &\multirow{3}{*}{48.71}  & \multirow{3}{*}{\textbf{75.43}}&
	  \textit{producer(x,y)} $\Leftarrow$ \textit{director(x,y)} \\ 
	   &&&&&&& \textit{producer(x,y)} $\Leftarrow$ \textit{screenwriter(x,y)}\\
	   &&&&&&& \textit{producer(x,y)} $\Leftarrow$ \textit{cast\_member(x,y)}\\
	   \hline

					
% 		\multirow{2}{*}{residence}  & \multirow{2}{*}{0.57} &\multirow{2}{*}{\textbf{48.0}}& \multirow{2}{*}{46.29} &
%     \multirow{2}{*}{0.43} &\multirow{2}{*}{0.43}& \multirow{2}{*}{47.71} 
% 		& \textit{residence(x,y)} $\Leftarrow$ \textit{place\_of\_birth(x,y)}\\ 
% 		&&&&&&& \textit{residence(x,y)} $\Leftarrow$ \textit{place\_of\_death(x,y)}\\
% 	\hline


	  % after\_a\_work\_by & 0.14	& \textbf{56.32}	& 56.32	& 0.14& 	0.29& 	53.02  & \textcolor[rgb]{0.88,0.31,0.04}{ \textit{screenwriter(x,y)} } $\Rightarrow$ \textit{producer(x,y)}\\ 
	  % \hline
	 

	  % work\_location & 1.14	& 69.57	& 62.57&	0.29	&0.57	&\textbf{69.86}& 
	  % \textit{field\_of\_work(x,y)} $\Leftarrow$ \textit{occupation(x,y)}\\ 
   %    \hline
		
% 	  developer&46.57	&52.14	&51.34	& 52.71	&54.00 &\textbf{54.71}&
% 	  \textit{distributor(x,y)}  $\Leftarrow$ \textit{developer(x,y)} $\wedge$  \textit{publisher(x,y)} \\ 
%       \hline

    

	  % field\_of\_work & 20.43	&23.32	&26.0	&21.71	&21.14	&\textbf{29.71}&
	  % \textit{field\_of\_work(x,y)} $\Leftarrow$ \textit{occupation(x,y)}\\ 
   %    \hline


	
	   \multirow{2}{*}{mother} & \multirow{2}{*}{63.72 }
      &\multirow{2}{*}{40.45} & \multirow{2}{*}{65.57}
      &\multirow{2}{*}{41.14} 
      &\multirow{2}{*}{44.43} & \multirow{2}{*}{\textbf{74.29}}
	  &\textit{mother(x,z)} $\Leftarrow$ \textit{spouse(x,y)} $\wedge$ \textit{father(y,z)}\\ 
			  &&&&&&& \textit{mother(x,y)}   $\Leftarrow$ \textit{child(y,x)}\\ 
      \hline

  	  nominated\_for  & 97.57&	97.14	&97.14&	98.00	&\textbf{98.14}&	97.43&
  	  \textit{nominated\_for(x,z)} $\Leftarrow$ \textit{award\_received(x,y)} $\wedge$ \textit{winner(y,z)}  \\ 
	  \hline	  

    %   \multirow{2}{*}{lyrics\_by} & \multirow{2}{*}{0.00 }
    %   &\multirow{2}{*}{71.48} & \multirow{2}{*}{71.79}
    %   &\multirow{2}{*}{0.00} 
    %   &\multirow{2}{*}{0.00} & \multirow{2}{*}{\textbf{72.05}}
    %   &  \textit{lyrics\_by(x,y)} $\Leftarrow$ \textit{composer(x,y)} \\
    %   &&&&&&& \textit{lyrics\_by(x,y)} $\Leftarrow$ \textit{perfomer(x,y)}\\
    %   \hline
      


% 	  connecting\_line&0.00 & 30.0 &\textbf{34.14} & 0.00	 & 0.00 & 	28.43 & 
%       \textit{connecting\_line(x,z)} $\Leftarrow$ \textit{adjacent\_station(y,x)} $\wedge$ \textit{part of(y,z)} \\ 
    %   \hline

    %   drafted\_by& 0.00 & \textbf{97.75}&96.53 & 0.00	 & 0.00 & 	96.88 & 
    %   \textit{drafted\_by(x,z)} $\Leftarrow$ \textit{member\_of\_sports\_team(y,x)} \\ 
      
	  \Xhline{1.2pt} %添加表格底部粗线

	   
	\end{tabular}
	\caption{Comparison ConSE result with all different embeddings on F1 score, and meanwhile presenting related rules w.r.t unseen relations.
	}
	\label{rule table}
	\vspace{-3mm}
\end{table*}

==> tables/zsre-general.tex <==
\begin{table}[htb]
\label{zsre gzsl}
\centering
\small
\caption{The result of ZSRE under GZSL.}\label{ZSLE}
\linespread{1.3}\selectfont
\begin{tabular}{c|ccc|ccc}
% \hline
\Xhline{1.2pt}
			\hline
            &\multicolumn{3}{c|}{ConSE} &\multicolumn{3}{c}{DeViSE}\\
            \hline
            &$Hit_{1}^{S}$    &$Hit_{1}^{U}$  &$H_{1}$  &$Hit_{1}^{S}$  &$Hit_{1}^{U}$  &$H_{1}$ \\
\hline
$E_{wd}$    &74.17  &0.01   &0.02   &34.39  &0.31   &0.61 \\
$E_{kg}$    &69.40  &2.30   &4.45   &57.89  &6.71   &12.02\\
$E_{rl}$    &75.75  &\textbf{3.97}   &\textbf{7.54}   &52.78  &\textbf{8.18}  &\textbf{14.16}\\
\hline
$E_{wk}$ 	&78.90	&0.79	&1.56	&60.91	&3.80	&7.15\\
$E_{wr}$ 	&70.12	&1.02	&2.01	&55.37	&5.85	&10.58\\
$E_{kr}$ 	&68.49	&\textbf{4.44}	&\textbf{8.34}	&56.99	&\textbf{9.53}	&\textbf{16.33}\\
\Xhline{1.2pt}
% \hline
\end{tabular}
\end{table}


==> tables/zsre-traditional.tex <==
% \begin{table*}[!hbt]
% \center
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}

% \hline
%  & \multicolumn{3}{c|}{PCNN+ConSE} & \multicolumn{3}{c|}{PCNN+DeViSE} & \multicolumn{3}{c|}{BERT+ConSE} & \multicolumn{3}{c|}{BERT+DeViSE} \\
% \hline 
% &    $Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &  $Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &$Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &$Hit_1^S$    &    $Hit_1^U$      &     $H_1$ \\
% \hline
% $E_{wd}$&          &          &          &           &          &          &          &          &          &           &          &       \\ 
% \hline 

% $E_{kg}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{rl}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{wk}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{wr}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{kr}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 
% \end{tabular}
% \end{table*}

\begin{table}[htb]
\label{zsre_tzsl}
\centering
\small
\caption{The result of ZSRE under TZSL.}
\linespread{1.3}\selectfont
\begin{tabular}{c|ccc|ccc}

\Xhline{1.2pt}
% \hline
            &\multicolumn{3}{c|}{ConSE}  &\multicolumn{3}{c}{DeViSE} \\
            \hline
            &$Hit_{1}$  &$Hit_{2}$  &$Hit_{5}$    &$Hit_{1}$  &$Hit_{2}$  &$Hit_{5}$ \\
\hline
$E_{wd}$    &18.23  &24.55  &38.87  &16.85  &25.31  &40.33 \\
$E_{kg}$    &36.91  &50.37  &66.00  &26.54  &39.89  &63.41 \\
$E_{rl}$    &\textbf{37.37}  &\textbf{53.06}  &\textbf{69.45} &\textbf{29.56}  &\textbf{44.04}  &\textbf{64.33} \\
\hline
$E_{wk}$ 	&24.12	&39.48	&60.82	&23.72	&36.97	&59.90 \\
$E_{wr}$ 	&31.63	&42.17	&62.97	&27.21	&41.43	&61.48 \\
$E_{kr}$ 	&\textbf{38.59}	&\textbf{53.86}	&\textbf{69.78}	&\textbf{32.27}	&\textbf{47.73}	&\textbf{67.5}	\\
\Xhline{1.2pt}
% \hline
\end{tabular}
\end{table}


==> tables/zsre.tex <==
% \begin{table*}[!hbt]
% \center
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}

% \hline
%  & \multicolumn{3}{c|}{PCNN+ConSE} & \multicolumn{3}{c|}{PCNN+DeViSE} & \multicolumn{3}{c|}{BERT+ConSE} & \multicolumn{3}{c|}{BERT+DeViSE} \\
% \hline 
% &    $Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &  $Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &$Hit_1^S$    &    $Hit_1^U$      &     $H_1$  &$Hit_1^S$    &    $Hit_1^U$      &     $H_1$ \\
% \hline
% $E_{wd}$&          &          &          &           &          &          &          &          &          &           &          &       \\ 
% \hline 

% $E_{kg}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{rl}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{wk}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{wr}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 

% $E_{kr}$&          &          &          &           &          &          &          &          &          &           &          &       \\  
% \hline 
% \end{tabular}
% \end{table*}

\begin{table*}[htb]
\label{zsre}
\centering
\caption{The result of ZSRE under TZSL and GZSL with diffrent relational representations.}\label{ZSLE}
\linespread{1.3}\selectfont
\begin{tabular}{c|ccc|ccc||ccc|ccc}

\Xhline{1.2pt}
			\multirow{3}{*}{}&\multicolumn{6}{c||}{TZSL}    &\multicolumn{6}{c}{GZSL}  \\
			\hline
            &\multicolumn{3}{c|}{ConSE}  &\multicolumn{3}{c||}{DeViSE}   &\multicolumn{3}{c|}{ConSE}    
            &\multicolumn{3}{c}{DeViSE}\\
            \hline
            &$Hit_{1}$  &$Hit_{2}$  &$Hit_{5}$    &$Hit_{1}$  &$Hit_{2}$  &$Hit_{5}$ &$Hit_{1}^{S}$    &$Hit_{1}^{U}$  &$H_{1}$  &$Hit_{1}^{S}$  &$Hit_{1}^{U}$  &$H_{1}$ \\
\hline
$E_{wd}$    &18.23  &24.55  &38.87  &16.85  &25.31  &40.33 &74.17  &0.01   &0.02   &34.39  &0.31   &0.61 \\
$E_{kg}$    &36.91  &50.37  &66.00  &26.54  &39.89  &63.41 &69.40  &2.30   &4.45   &57.89  &6.71   &12.02\\
$E_{rl}$    &37.37  &53.06  &69.45  &29.56  &44.04  &64.33 &75.75  &3.97   &7.54   &52.78  &8.18   &14.16\\
\hline
$E_{wk}$ 	&24.12	&39.48	&60.82	&23.72	&36.97	&59.9	&78.9	&0.79	&1.56	&60.91	&3.8	&7.15\\
$E_{wr}$ 	&31.63	&42.17	&62.97	&27.21	&41.43	&61.48	&70.12	&1.02	&2.01	&55.37	&5.85	&10.58\\
$E_{kr}$ 	&38.59	&53.86	&69.78	&32.27	&47.73	&67.5	&68.49	&4.44	&8.34	&56.99	&9.53	&16.33\\
\Xhline{1.2pt}
\end{tabular}
\end{table*}

